Incorporating Task-specific Concept Knowledge into Script Learning

In this paper, we present Tetris, a new task of Goal-Oriented Script Completion. Unlike previous work, it considers a more realistic and general setting, where the input includes not only the goal but also additional user context, including preferences and history. To address this problem, we propose a novel approach, which uses two techniques to improve performance: (1) concept prompting, and (2) script-oriented contrastive learning that addresses step repetition and hallucination problems. On our WikiHow-based dataset, we find that both methods improve performance. The dataset, repository, and models will be publicly available to facilitate further research on this new task.

==> 3dataset.tex <==
\section{Dataset}
\label{sec:data}


% \begin{table}
% 	\centering
% 	\begin{tabular}{lllll}
% 		\toprule
% 		Setting &Anno.& \#Doc.& \#Sent. & \#Mention   \\
% 		\midrule
% 		Train &Distant&    80&6565&10318\\
% 		Dev &Human&20&520&1118\\
% 		Test&Human&            20&663&1295 \\
% 		\bottomrule
% 	\end{tabular}
% 	\caption{Dataset Statistics for CHEMET}
% 	\label{datastats}
% \end{table}
\begin{table*}[]\begin{small}
\centering
\begin{tabular}{l|l|l|l}
\toprule

 & Food and Entertaining & Finance and Business & Cars \& Other Vehicles \\ \hline
\# Train Samples & 10600 & 2824 & 2214 \\
\# Dev Samples & 3449 & 873 & 741 \\
\# Test Samples & 3567 & 930 & 714 \\
\# Articles & 2201 & 802 & 481 \\
Avg \# Tokens/Step & 8.66 & 7.25 & 9.31 \\
Avg \# Steps/Article & 10.42 & 8.66 & 10.41 \\\bottomrule
\end{tabular}
\caption{Statistics summarizing the WikiHow dataset.}
\label{tab:data-stats}
\end{small}
\end{table*}
% \begin{table}
% \begin{tabular}{llll}
% \hline
%      & Food and Entertaining & Finance and Business & Cars \& Other Vehicles \\ \hline
%     \# Train Samples & 10600 & 2824 & 2214 \\
%     \# Dev Samples & 3449 & 873 & 741 \\
%     \# Test Samples & 3567 & 930 & 714 \\
%     \# Articles & 2201 & 802 & 481 \\
%     Avg \# Tokens/Step & 9 & 7 & 9 \\
%     Avg \# Steps/Article & 10 & 9 & 10
% \end{tabular}
% \caption{Statistics summarizing the WikiHow dataset.}
% \label{tab:data-statss}
% \end{table}

<intro wikihow> We collect data from Wikihow a 
each wikiHow article contains a high-level goal and one or more different methods2 to achieve it. Each method then includes a series of specific steps, typically accompanied with corresponding images.

Each article contains: main bodies of texts (titles, methods/parts, headers, d
An example is shown in Figure 1. The dataset contain 15000 instructional articles, each containing a title/\textit{goal} and multiple sections, each section contains a section header/\textit{subgoal} (describing what is going on in this section) and \textit{steps}. 



<talk stats, as shown in Table 1, the corpus consists of 53,189 wikiHow

<filtering, 
structure 
to task , so we combine


\subsection{Dataset}
We evaluate SEE on a dataset we construct from Wikihow. 

Since we consider the low-resource regime in our study, we simulate it by moving out 80\% of the data as the ``web'' of instruction text, which reflects the web in real-life for which it requires too much computing resource to be used a training data.

For the rest of the data, we split it by the train-dev-test ratio of 6-2-2. 
